A Fault Analysis on SNOVA

SNOVA is a post-quantum cryptographic signature scheme known for its efficiency and compact key sizes, making it a second-round candidate in the NIST post-quantum cryptography standardization process. This paper presents a comprehensive fault analysis of SNOVA, focusing on both permanent and transient faults during signature generation. We introduce several fault injection strategies that exploit SNOVA's structure to recover partial or complete secret keys with limited faulty signatures. Our analysis reveals that as few as 22 to 68 faulty signatures, depending on the security level, can suffice for key recovery. We propose a novel fault-assisted reconciliation attack, demonstrating its effectiveness in extracting the secret key space via solving a quadratic polynomial system. Simulations show transient faults in key signature generation steps can significantly compromise SNOVA's security. To address these vulnerabilities, we propose a lightweight countermeasure to reduce the success of fault attacks without adding significant overhead. Our results highlight the importance of fault-resistant mechanisms in post-quantum cryptographic schemes like SNOVA to ensure robustness.

==> app_code.tex <==
\section{Implementation from SNOVA}
\label{app:code}
Here we present the code snipets that we used in the paper. 

\begin{lstlisting}[language=C, label={lst:mul},  caption={C code to perform multiplication in $\FF_{16}$}]
uint8_t mul(uint8_t a, uint8_t b){
    uint8_t r = ((a) << 4) ^ (b);
    return mt4b[r];
}
\end{lstlisting}

\begin{lstlisting}[language={[x86masm]Assembler}, label={lst:asm}, caption={Assembly code to perform multiplication in $\FF_{16}$}]
mul(unsigned char, unsigned char):
        push    {r7}
        sub     sp, sp, #20
        add     r7, sp, #0
        mov     r3, r0
        mov     r2, r1
        strb    r3, [r7, #7]
        mov     r3, r2
        strb    r3, [r7, #6]
        ldrsb   r3, [r7, #7]
        lsls    r3, r3, #4
        sxtb    r2, r3
        ldrsb   r3, [r7, #6]
        eors    r3, r3, r2
        sxtb    r3, r3
        strb    r3, [r7, #15]
        ldrb    r3, [r7, #15]   @ zero_extendqisi2
        ldr     r2, .L7
        ldrb    r3, [r2, r3]    @ zero_extendqisi2
        mov     r0, r3
        adds    r7, r7, #20
        mov     sp, r7
        ldr     r7, [sp], #4
        bx      lr
.L7:
        .word   _ZL4mt4b
\end{lstlisting}

\begin{lstlisting}[language=C, caption={Code snippet in C for the generation of the vinegar values}, label={lst:gen_of_vinegar}]
memcpy(vinegar_input, pt_private_key_seed, SEED_LENGTH_PRIVATE_KEY);
memcpy(vinegar_input + SEED_LENGTH_PRIVATE_KEY, digest, 64);
memcpy(vinegar_input + (SEED_LENGTH_PRIVATE_KEY + bytes_digest), array_salt, BYTES_SALT);
int num_sign = 0;
int flag_redo = 0;
do {
    vinegar_input[SEED_LENGTH_PRIVATE_KEY + bytes_digest + BYTES_SALT] = num_sign;
    shake256(vinegar_input,
             SEED_LENGTH_PRIVATE_KEY + bytes_digest + BYTES_SALT + 1,
             vinegar_in_byte, (v_SNOVA * lsq_SNOVA + 1) >> 1);

    for (int index = 0; index < v_SNOVA; index++) {
            for (int i = 0; i < RANK; ++i) {
                for (int j = 0; j < RANK; ++j) {
                    if(counter & 1){
                        set_gf16m(X_in_GF16Matrix[index], i, j, (vinegar_in_byte[counter >> 1] >> 4));
                    }
                    else
                    {
                        set_gf16m(X_in_GF16Matrix[index], i, j, (vinegar_in_byte[counter >> 1] & 0xF));
                    }
                    counter++;
                }
            }
        }
} while (flag_redo);
\end{lstlisting}



==> app_grover.tex <==
\section{Adapting Grover's Algorithm to SNOVA reconciliation quadratic system}
\label{app:grover}

Grover's algorithm is a quantum search algorithm that provides a quadratic speedup for unstructured search problems. It finds a marked item in an unsorted database of \(N\) items with high probability using \(O(\sqrt{N})\) queries to the database. We  present two cases, when one directly apply Grover's algorithm against SNOVA reconciliation quadratic system, and the scenarios presented in Section~\ref{sec:exploit}. First, let us remind the reader about Grover's algorithm. 

\subsubsection{Algorithm Description}
Consider a database of \(N\) items and a function \(f: \{0, 1, \ldots, N-1\} \to \{0, 1\}\) that identifies the marked item(s) \(x^*\) such that:
\[
f(x) = \begin{cases}
1 & \text{if } x = x^*, \\
0 & \text{otherwise}.
\end{cases}
\]

Grover's algorithm consists of the following steps:

\begin{enumerate}
    \item \textbf{Initialization:}
    Prepare the quantum state in an equal superposition of all possible states:
    \[
    |\psi\rangle = \frac{1}{\sqrt{N}} \sum_{x=0}^{N-1} |x\rangle
    \]

    \item \textbf{Oracle:}
    Apply the oracle \(O_f\), which flips the phase of the marked state \(x^*\):
    \[
    O_f|x\rangle = \begin{cases}
    -|x\rangle & \text{if } f(x) = 1, \\
    |x\rangle & \text{otherwise}.
    \end{cases}
    \]

    \item \textbf{Diffusion Operator:}
    Apply the Grover diffusion operator \(D\), defined as:
    \[
    D = 2|\psi\rangle \langle \psi| - I
    \]
    which inverts the amplitude of each state about the mean amplitude.

    \item \textbf{Iteration:}
    Repeat the application of the oracle and the diffusion operator \(O(\sqrt{N})\) times.

    \item \textbf{Measurement:}
    Measure the quantum state. The result will be the marked item \(x^*\) with high probability.
\end{enumerate}

\subsubsection{Mathematical Formulation}
The combined operation of the oracle and the diffusion operator is called a Grover iteration \(G\):
\[
G = D O_f
\]
Each iteration amplifies the amplitude of the marked state. After \(O(\sqrt{N})\) iterations, the probability of measuring the marked state is close to 1.


\subsection{Quantum-assisted search}
 We here demonstrate how Grover's algorithm can be used to solve SNOVA reconciliation quadratic system more efficiently. From Section \ref{sec:exploit} we already have some information that we acquire from the side-channel attack. 
 In that section two scenarios are presented. On the one hand, for the first scenario, one tries to recover the missing bits by solving the resulting  quadratic system over \(\mathbb{F}_{2}\) given the partial-but-perfect bit information gained from the side-channel attack.
 On the other hand, for the second scenario, one uses the partial-but-imperfect bit information to launch an enumeration algorithm that uses Grover's algorithm. In both cases, one can directly apply the oracle construction from~\cite{10.1007/978-3-319-49445-6_17} and perform a quantum-assited search, Table~\ref{tab:quantum_resources} shows the costs.
 %\todo[]{add a table with resources for scenario 1 and 2} 

\begin{table}[htp]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c@{\hskip 1em}c@{\hskip 1em}c@{\hskip 1em}c@{\hskip 1em}c@{\hskip 1em}c@{\hskip 1em}c}
    \toprule 
         & & $85\%$ & $90\%$ & $95\%$ & $(4lv, 4ml^2)$ \\ 

       $(v, o, q, l)$ & \#eqs  & (Qubits, Gates) & (Qubits, Gates) & (Qubits, Gates) & (Qubits, Gates) \\ \midrule 
     (37, 17, 16, 2) & 272 & (67, $10^{8.3}$) & (52, $10^{8.0}$) & (37, $10^{7.6}$) & (272, $10^{9.5}$)\\
     (25, 8, 16, 3) & 288 & (67, $10^{8.3}$) & (52, $10^{8.0}$) & (37, $10^{7.6}$) & (288, $10^{9.6}$)\\
     (24, 5, 16, 4) & 320 & (80, $10^{8.7}$) & (61, $10^{8.4}$) & (42, $10^{7.9}$) & (320, $10^{9.7}$)\\
     (56, 25, 16, 2) & 400 & (90, $10^{8.8}$) & (67, $10^{8.3}$) & (45, $10^{7.8}$) & (400, $10^{9.8}$)\\
     (49, 11, 16, 3) & 396 & (111, $10^{9.1}$) & (81, $10^{8.6}$) & (52, $10^{8.0}$) & (396, $10^{9.9}$)\\
     (37, 8, 16, 4) & 512 & (111, $10^{9.0}$) & (82, $10^{8.6}$) & (52, $10^{8.0}$) & (512, $10^{10.0}$)\\
     (75, 33, 16, 2) & 528 & (112, $10^{9.0}$) & (82, $10^{8.6}$) & (52, $10^{8.0}$) & (528, $10^{10.1}$)\\
     (66, 15, 16, 3) & 540 & (141, $10^{9.3}$) & (102, $10^{8.8}$) & (62, $10^{8.2}$) & (540, $10^{10.2}$)\\
     (60, 10, 16, 4) & 640 & (166, $10^{9.5}$) & (118, $10^{9.0}$) & (70, $10^{8.3}$) & (640, $10^{10.3}$)\\
       
    \bottomrule
    \end{tabular}
    }
    \caption{Quantum resource estimates (qubits and gates) for constructing the MQ oracle using Grover's algorithm. The gate counts are logarithmic estimations based on the complexity of Toffoli gate implementations and based on the results from \cite{10.1007/978-3-319-49445-6_17}.}
    \label{tab:quantum_resources}
\end{table}
\iffalse % I think this repetition should be out. 
The second scenario refers to the setting where the attacker uses information produced by an imperfect attack. Here, the adversary finds some, but insufficient, side-channel information about the target secret. Consequently, the attacker must enumerate and test candidates for the target secret (in some order along with a decision oracle) to determine whether a candidate is correct \cite{cryptoeprint:2018/019}. This scenario became achievable after the work of Veyrat-Charvillon et al.~\cite{10.1007/978-3-642-35999-6_25}. 

We assume that the side-channel attack returns a score vector per value \(\texttt{V}_{i,j\beta}\), for \(i \in [v], j \in [l]\) and fixed \(\beta \in [l]\). A side-channel attack takes in a set of leakages (of size \(N_{\ell}\), where \(N_{\ell}\) might be as low as one) and returns the output of a function termed a distinguisher in the side-channel literature. There are many techniques for side-channel analysis using different types of distinguishers, resulting in different scores (see \cite{10.5555/1208234} for an overview). Here, we deal with distinguishers that produce additive scores indicating likelihood values.

More concretely, we can obtain \(v \cdot l\) lists, where the list \(\widetilde{\texttt{L}}_{ij}\) contains at most \(2^{N_{\text{bits}}}\) 2-tuples of the form \((\texttt{score}, \texttt{value})\). The first component \(\texttt{score}\) is a real number (candidate score) and the second component \(\texttt{value}\) is a \(N_{\text{bits}}\)-bit string (candidate value); \(\texttt{score}\) represents how likely \(\texttt{value}\) is the correct value for the corresponding entry \(\texttt{V}_{i,j,\beta}\).
\fi
%\todo[]{In the scenario two, there is nothing known so the attacker  has to retrieve $n_{bits}lv$ bits by using the enumeration algorithm. Please add that to the table too.}
%\todo{The problem is that I do not see a way of writing properly, I understand that we will have a list but I don't know how we are doing this with grover's algorithm} 

%Hi Gustavo
%are you here?

%If so, you only have to provide an oracle for $T$ defined in Equation 5. The enumeration is essentially the same algorithm we propose in the previous paper.

%$T$ is a quadratic system on 4lv variables and $4ml^2$ equations


%Ok, I will try to find this oracle.. I am just having some problem to really quantify for the scenario 2. Ok! It is the same as you did for the first scenario. Ok, :) simply add a column to the table!
%I made a python script that compute the costs, I will add in a folder here


 However, we can potentially extend Grover's algorithm to directly target the reconciliation quadratic system over $\mathbb{F}_{16}$. Recall that a reconciliation attack on SNOVA, when considered over the underlying field, is as an attack on the induced $(lv, lo, q)$ UOV instance \cite{cryptoeprint:2020/1343,cryptoeprint:2024/096,cryptoeprint:2024/110}, whose goal is to try to find a vector $\mathbf{u} \in \mathcal{O}$, where $$\mathcal{O}:=T^{-1}(\{x =(x_1,\ldots,x_{ln}) \in \mathbb{F}^{ln}_q :x_1=\ldots =x_{lv} =0\}).$$Thus, it requires finding an element $\mathbf{u}_0 = (u_1 , \ldots,u_{lv} ,0,\ldots,1)^t \in \mathbb{F}_q^{ln}$ such that 



\begin{equation}
   \label{rec} \mathbf{u}_0^t([\Lambda_{S^{j}}][P_i][\Lambda_{S^{k}}])\mathbf{u}_0=0 \in \mathbb{F}_q,
\end{equation}for~$i \in [m],j,k \in \{0,1,\ldots, l-1\}$. This is a quadratic system with $l^2m$ equation on $lv$ unknowns. Also, each $\mathbf{u}\in \{\mathbf{u}_0, [\Lambda_{S^{1}}]\mathbf{u}_0,[\Lambda_{S^{2}}]\mathbf{u}_0, \ldots, [\Lambda_{S^{l-1}}]\mathbf{u}_0\}$ will also satisfy Eq. (\ref{rec}), and they are linearly independent. In order for the attacker to get the rest of vectors in the secret space $\mathcal{O}$, he can use the equation Eq(\ref{a}), which gives a linear system with $2ol^2$ equations on $ln$ unknowns. 

\paragraph{Problem Definition}
The reconciliation quadratic system in SNOVA consists of \(ml^2\) quadratic equations in \(lv\) variables over \(\mathbb{F}_{16}\):
\[
P_i(x_1, x_2, \ldots, x_{lv},\ldots,1) = 0, \quad x_i \in \mathbb{F}_{16}, \quad i = 1, 2, \ldots, ml^2
\]

\paragraph{Quantum Representation}
Each variable \(x_i\) is represented by 4 qubits:
\[
|x_i\rangle = |x_{i0}x_{i1}x_{i2}x_{i3}\rangle
\]
For \( lv\) variables, this requires \(4lv\) qubits.

\paragraph{Oracle Construction}
The oracle \(O_f\) checks the MQ equations and flips the phase of satisfying states:
\[
O_f |x\rangle = \begin{cases}
-|x\rangle & \text{if } f_1(x) = 0 \text{ and } \ldots \text{ and } f_{ml^2}(x) = 0 \\
|x\rangle & \text{otherwise}
\end{cases}
\]

\paragraph{Field Operations}
Addition and multiplication in \(\mathbb{F}_{16}\) are implemented using quantum circuits that perform polynomial arithmetic modulo \(x^4 + x + 1\).

\paragraph{Grover's Algorithm}
\begin{enumerate}
    \item Initialize the quantum state:
    \[
    \frac{1}{\sqrt{16^{lv}}} \sum_{x \in \mathbb{F}_{16}^{lv}} |x\rangle
    \]
    \item Apply the oracle \(O_f\).
    \item Apply the Grover diffusion operator.
    \item Repeat \(\Theta(4^{lv})\) times.
\end{enumerate}

\paragraph{Quantum Circuit Example}
\[
\Qcircuit @C=1em @R=.7em {
  \lstick{|x_0\rangle} & \qw & \multigate{3}{O_f} & \qw & \rstick{|x_0\rangle} \qw \\
  \lstick{|x_1\rangle} & \qw & \ghost{O_f} & \qw & \rstick{|x_1\rangle} \qw \\
  \lstick{|x_2\rangle} & \qw & \ghost{O_f} & \qw & \rstick{|x_2\rangle} \qw \\
  \lstick{|x_3\rangle} & \qw & \ghost{O_f} & \qw & \rstick{|x_3\rangle} \qw \\
}
\]

Using Grover's algorithm to directly solve the SNOVA reconciliation equation significantly reduces the time complexity of the underlying MQ problem from \(\Theta(16^{lv})\) to \(\Theta(4^{lv})\). One open problem is how to build the oracle \(O_f\); that is, one still needs to analyze the resources required for the field arithmetic and compute the full costs of implementing the oracle.

==> conclusion.tex <==
In this paper, we provide a comprehensive analysis of side-channel attacks against SNOVA. Our novelty lies in the algorithms that handle leaked data and faulty signatures. In the first case, we present two scenarios where an attacker can use our algorithms to recover the secret key. Regarding the fault attack analysis, we demonstrate that only a small number of faulty signatures are needed to partially recover the SNOVA secret key. More precisely, we show that one fixed value in the vinegar part allows an attacker to collect $lo+2$ signatures. In Table~\ref{tab:parameters}, an attacker only needs to produce $22$, $34$, and $42$ signatures for security levels I, III, and V, respectively.

We believe our attacks could potentially be adapted to other UOV signatures, since they share a similar structure. For example, a potential next target could be MAYO~\cite{mayo}, which is built on the same UOV paradigm, though it would require modifications to our algorithms. Additionally, a deeper analysis would be needed for quantum enumeration since we only briefly discuss it, and the oracle for MAYO needs to be developed.

==> fault_analysis.tex <==
%\rv[inline]{ I think this section will serve as a prelude to our fault attacks. Basically here we can show a deep analysis whose goal is to show potential points within the signing algorithm that may lead to a key recovery if a fault is set. Clearly at the end of this section, we should identify the point we exploit in the Section \ref{sec:fault}. Does this section make sense to you?}

%\gb[inline]{I think that we can add this section I understand that you want to point it as like, well we did an analysis and we found X, Y, and Z. I guess that it makes sense to say, we did not focus only on one attack, we did a proper analysis of it}

%\rv[inline]{yes, that's the point of this section. However, I do not know if that analysis makes a whole section. Let's write it and then we can decide if it makes sense to merge this section with the next one.}
 



==> sca_q.tex <==

In our examination of SNOVA, potential leaks in the 
instructions have been identified. This section delves into 
further sources of leakage that play a role in key recovery.
Our attention is particularly drawn to the computation of 
the vinegar part, a focal point addressed in~\cite{Aulbach_Campos_Krämer_Samardjiska_Stöttinger_2023} 
within the context of the UOV scheme. It is worth noting that
 additional studies, such as~\cite{Park_Shim_Koo_Han_2018,9474157},
underscore side-channel attacks on UOV and Rainbow schemes utilizing correlation power analysis.
\subsection{Structure of SNOVA}


Let us delve into the intricacies of SNOVA~\cite{cryptoeprint:2024/096,cryptoeprint:2024/110,cryptoeprint:2022/1742}.
Recall that the SNOVA public map is given by $\widetilde{P}=[\widetilde{P}_1,\cdots ,\widetilde{P}_{m}]:\mathcal{R}^n \rightarrow \mathcal{R}^m$, where 

$$ \widetilde{P}_i(\mathbf{U}) = \sum_{\alpha=1}^{l^2} \sum_{d_j=1}^{n} \sum_{d_k=1}^{n} A_{\alpha} U^t_{d_j}(Q_{\alpha1}P_{i,d_{j}d_{k}}Q_{\alpha 2})U_{d_k}\cdot B_{\alpha}$$

\noindent with the variable $\mathbf{U} = (U_1, \ldots , U_{n})^t$ and $$[P_i]=\begin{bmatrix}
P_i^{11} & P_i^{12} \\
P_i^{21} & P_i^{22}
\end{bmatrix}=[T]^{t}[F_i][T]=\begin{bmatrix}I_{v \times v}&  O\\
(T_{v \times o})^{t}& I_{o \times o}
\end{bmatrix}\begin{bmatrix}
F_i^{11} & F_i^{12} \\
F_i^{21} & O\\
\end{bmatrix}\begin{bmatrix}I_{v \times v}& T_{v \times o}\\
O& I_{o \times o}
\end{bmatrix},$$ where $A_{\alpha},B_{\alpha} $ are invertible elements chosen randomly from $\mathcal{R}$, and $Q_{\alpha 1},Q_{\alpha 2}$ are invertible elements chosen randomly from $\mathbb{F}_{q}[S]$. We know that $$ \widetilde{P}_i(\mathbf{U}) = \sum_{\alpha=1}^{l^2}  A_{\alpha} \mathbf{U}^{t}([\Lambda_{Q_{\alpha1}}][P_{i}][\Lambda_{Q_{\alpha2}}]) \mathbf{U}\cdot B_{\alpha}.$$ 

Let us now consider the $(lv, lo,q)$ induced UOV instance given by $[P_i], [F_i], [T]$ over $\mathbb{F}_q$ and define $\mathcal{O}_1=\{x =(x_1,\ldots,x_{ln}) \in \mathbb{F}^{ln}_q :x_1=\ldots =x_{lv} =0\} \subset \mathbb{F}_q^{ln}.$ $\mathcal{O}_1$ has dimension 
$ol$ and furthermore $\mathbf{v}^t[F_i]\mathbf{u}=0$ for any $\mathbf{u},\mathbf{v} \in \mathcal{O}_1$. For key recovery attacks against UOV scheme and its variants, one has 
the task to find the oil space $\mathcal{O}=T^{-1}(\mathcal{O}_1)$ with  $dim_{\mathbb{F}_q} \mathcal{O}=lo$. Similarly for the SNOVA case,  an attacker has to find the oil space of the public map 
$T^{-1}(\{\mathbf{x} \in \mathcal{R}^{n}: x_1=x_2=\cdots=x_{v}=0 \})$.




\remark{ 
For any $\mathbf{u},\mathbf{v} \in \mathcal{O}$, $ 0\leq j,k \leq l-1$ we have 
\begin{equation}
   \label{a} \mathbf{v}^t([\Lambda_{S^{j}}][P_i][\Lambda_{S^{k}}])\mathbf{u}=0 \in \mathbb{F}_q ~\textrm{for}~i \in [m].
\end{equation}} 
\begin{proof}
Let $Q \in \mathbb{F}_{q}[S]$. Note that
\begin{align*}
[T] [\Lambda_{Q}]=&\begin{bmatrix}
Q  & 0 & \ldots& T_{0 v}Q& \ldots& T_{0 (n-1)}Q \\
0  & Q & \ldots& T_{1 v}Q & \ldots& T_{1 (n-1)}Q \\
\vdots & \vdots& \vdots & \vdots &\vdots & \vdots \\
0  & 0 & \ldots& Q & \ldots& 0 \\
\vdots & \vdots& \vdots & \vdots &\vdots & \vdots \\
0  & 0 & \ldots&  0 & \ldots& Q \\
\end{bmatrix}=\begin{bmatrix}
Q & 0 & \ldots& Q T_{0 v}& \ldots& QT_{0 (n-1)} \\
0  & Q & \ldots& Q T_{1 v} & \ldots& QT_{1 (n-1)} \\
\vdots & \vdots& \vdots & \vdots &\vdots & \vdots \\
0  & 0 & \ldots& Q & \ldots& 0 \\
\vdots & \vdots& \vdots & \vdots &\vdots & \vdots \\
0  & 0 & \ldots&  0 & \ldots& Q \\
\end{bmatrix}= [\Lambda_{Q}][T]
\end{align*} since $T_{i_1j_1},Q\in \mathbb{F}_{q}[S]$, and all elements in $\mathbb{F}_{q}[S]$ commute and they are symmetric. 
Also, $\Lambda_{Q}$ is symmetric. Therefore, 
\begin{align*}
  \mathbf{v}^t([\Lambda_{S^j}][P_i][\Lambda_{S^k}])\mathbf{u} =\mathbf{v}^t([\Lambda_{S^j}][T]^t[F_i][T][\Lambda_{S^k}])\mathbf{u}= \mathbf{v}^t[T]^t([\Lambda_{S^j}][F_i][\Lambda_{S^k}])[T]\mathbf{u}=0.
\end{align*} In other words, $([\Lambda_{S^j}][P_i][\Lambda_{S^k}])\mathcal{O} \subset \mathcal{O}^{\perp}$. Moreover, 
for any $A, B \in \mathbb{F}_{q}[S]$, we have that $A=\sum _{j=0}^{l-1}a_jS^{j}$ and $B=\sum _{k=0}^{l-1}b_kS^{k}$, for some $a_{j},b_{k} \in \mathbb{F}_q$, and therefore

\begin{align*}
   \mathbf{v}^t([\Lambda_{A}][P_i][\Lambda_{B}])\mathbf{u}=
   \mathbf{v}^{t} \big (\sum_{j=0}^{l-1}a_j [\Lambda_{S^{j}}] \big )[P_{i}]  \big (\sum_{k=0}^{l-1}b_k [\Lambda_{S^{k}}] \big ) )\mathbf{u}=\\
   \sum_{j=0}^{l-1}\sum_{k=0}^{l-1}\mathbf{v}^{t} [\Lambda_{a_j S^{j}}] [P_{i}][\Lambda_{ b_k S^{k}}] \mathbf{u}=0 ~\textrm{for}~i \in [m]. 
\end{align*}
 $\square$
\end{proof}
\remark{ 
If we find a subspace $\mathcal{O}^{'} \subset  \mathbb{F}_{q}^{ln}$ with dimension $ol$ such that any elements $u, v \in \mathcal{O}^{'}$ satisfy equation \ref{a}, then for any 
\begin{equation}
\label{const}
   \mathbf{U} \in \mathcal{O}^{'} \otimes \mathbb{F}_q^{l} \in \{ \mathbf{u} \otimes \mathbf{e}^t \in \mathcal{R}^n: \mathbf{u} \in \mathcal{O}^{'}, \mathbf{e}\in \mathbb{F}_q^{l}   \} 
\end{equation} we have $\widetilde{P}_i(\mathbf{U} )=0$ for $i\in [m]$.}
\begin{proof}
    

Consider  $$ \widetilde{P}_i(\mathbf{U}) = \sum_{\alpha=1}^{l^2}  A_{\alpha} \mathbf{U}^{t}([\Lambda_{Q_{\alpha1}}][P_{i}][\Lambda_{Q_{\alpha2}}]) \mathbf{U}\cdot B_{\alpha}$$ where $\mathbf{U}= \begin{bmatrix}
\mathbf{u}_1 \\
\mathbf{u}_2 \\
\vdots\\
\mathbf{u}_{n} \\

\end{bmatrix}= \begin{bmatrix}
u_{11} & u_{12} & \cdots & u_{1(l)} \\
u_{21} & u_{22} & \cdots & u_{2(l)} \\
\vdots & \vdots & \vdots & \vdots \\
u_{(ln)1} & u_{(ln)2} & \cdots & u_{(ln)(l)} \\

\end{bmatrix} \in \mathcal{O}^{'} \otimes \mathbb{F}_q^{l} \leq \mathcal{R}^n.$ Because of the construction of $\mathcal{O}^{'} \otimes \mathbb{F}_q^{l}$, we have that each column $\mathbf{U}_{:i_1} =
\begin{bmatrix}
u_{1,i_1}  \\
 u_{2,i_1}  \\
\vdots  \\
 u_{ln,i_1} \\
\end{bmatrix} \in \mathcal{O}^{'}$, with $1\leq  i_1 \leq l$,  and hence $\mathbf{U}_{:i_1}^{t}([\Lambda_{Q_{\alpha1}}][P_i][\Lambda_{Q_{\alpha2}}]) \mathbf{U}_{:i_2} =0$ for all $1\leq i_1,i_2\leq l$. \\
$\square$
\end{proof}

\subsection{Reconciliation attack on the induced $(lv, lo,q)$ UOV instance.} \label{section_rec}

A reconciliation attack on SNOVA, when considered over the underlying field, is as an attack on the induced $(lv, lo, q)$ UOV instance~\cite{cryptoeprint:2020/1343,cryptoeprint:2024/096,cryptoeprint:2024/110,cryptoeprint:2022/1742}, whose goal is to try to find a vector $\mathbf{u}_0 \in \mathcal{O}$. Thus, it requires finding an element $\mathbf{u}_0 \in \mathbb{F}_q^{ln}$ such that 



\begin{equation}
   \label{rec} \mathbf{u}_0^t([\Lambda_{S^{j}}][P_i][\Lambda_{S^{k}}])\mathbf{u}_0=0 \in \mathbb{F}_q,
\end{equation}for~$i \in [m],j,k \in \{0,1,\ldots, l-1\}$. 


\remark{ From line \ref{sigcom} from Algorithm \ref{scheme:sign}, we know that for any valid signature $(\texttt{S}, \texttt{salt})$, it holds $\texttt{S} =[T]^{-1}\texttt{V}$, where $\texttt{V}=(\texttt{V}_1,\ldots,\texttt{V}_v,\texttt{O}_1, \ldots, \texttt{O}_o)^t$ and $[T]^{-1}=[T]$.Therefore, for any $1 \leq \beta \leq l$, we have 

$$ \begin{bmatrix}
\texttt{S}_{1,:\beta} \\
\vdots\\
\texttt{S}_{v,:\beta}\\
\vdots\\
\texttt{S}_{n,:\beta}\\
\end{bmatrix}=\begin{bmatrix}
1 & 0 & \ldots & 0&T^{12}_{1,1}&\ldots &T^{12}_{1,o} \\
\vdots & \vdots & \ddots & \vdots&\vdots &\ddots &\vdots \\
0 & 0 & \ldots & 1 & T^{12}_{v,1}&\ldots &T^{12}_{v,o} \\
\vdots & \vdots & \ddots & \vdots&\vdots &\ddots &\vdots \\
0 & 0 & \ldots & \ldots &0 &\ldots&1 \\
\end{bmatrix}\begin{bmatrix}
\texttt{V}_{1,:\beta}\\
\vdots\\
\texttt{V}_{v,:\beta}\\
\texttt{O}_{1,:\beta}\\
\vdots\\
\texttt{O}_{o,:\beta}\\
\end{bmatrix}=\begin{bmatrix}
\texttt{V}_{1,:\beta} - \sum_{j=1}^{o}T^{12}_{1j}\texttt{O}_{j,:\beta}\\
\vdots\\
\texttt{V}_{v,:\beta}- \sum_{j=1}^{o}T^{12}_{vj}\texttt{O}_{j,:\beta}\\
\texttt{O}_{1,:\beta}\\
\vdots\\
\texttt{O}_{o,:\beta}\\
\end{bmatrix}$$ where $\texttt{A}_{:\beta} \in \mathbb{F}_q^{l}$ denotes the $\beta$-th column of $\texttt{A}\in \mathbb{F}_q^{l\times l}$.} If  $\texttt{V}_{1,:\beta}, \ldots, \texttt{V}_{v,:\beta}$ are known by the attacker, then the attacker can set $$\mathbf{u}_0=\begin{bmatrix}
\texttt{S}_{1,:\beta} -\texttt{V}_{1,:\beta}\\
\vdots\\
\texttt{S}_{v,:\beta}-\texttt{V}_{v,:\beta}\\
\vdots\\
\texttt{S}_{n,:\beta}\\
\end{bmatrix}, $$ which will satisfy Eq. (\ref{rec}). Also, each $\mathbf{u}\in \{\mathbf{u}_0, [\Lambda_{S^{1}}]\mathbf{u}_0,[\Lambda_{S^{2}}]\mathbf{u}_0, \ldots, [\Lambda_{S^{l-1}}]\mathbf{u}_0\}$ will also satisfy Eq. (\ref{rec}), and they are linearly independent. In order for the attacker to get the rest of vectors in the secret space $\mathcal{O}$, he can use the equation Eq(\ref{a}), which gives a linear system with $2ol^2$ equations on $ln$ unknowns. Finally, once the attacker has recovered $\mathcal{O}$, he can use the construction given by Eq (\ref{const}) to get an equivalent SNOVA secret space.

The main task by the attacker is to find $\texttt{V}_{1,:\beta}, \ldots, \texttt{V}_{v,:\beta}$ for a valid signature $(\texttt{S}, \texttt{salt})$ and some $1 \leq \beta \leq l$. So a reasonable strategy by the attacker is trying to find a source of leakage during the computation of the vinegar part. In particular, the attacker may try to target the line \ref{compvin2} of Algorithm~\ref{scheme:sign}. According to the SNOVA specification~\cite{SNOVA}, the line \ref{compvin2} of Algorithm~\ref{scheme:sign} is computed by Algorithm~\ref{computevinegarpart}. In particular, the attacker may try to target the line either  \ref{linetarget1} or \ref{linetarget2} of Algorithm~\ref{computevinegarpart}, since $\{A_{\alpha},B_{\alpha}, Q_{\alpha1}, Q_{\alpha2}\}_{\alpha\in [l^2]}$ are public.


\begin{algorithm}[htp]  
\caption{Computes the vinegar part of the central map}
\label{computevinegarpart}
\begin{algorithmic}[1]

\STATE \textbf{function} $\texttt{compute\_vinegar\_part}(v,o, l,\{F_i^{11}\}_{i\in [m]}, \{A_{\alpha},B_{\alpha}, Q_{\alpha1}, Q_{\alpha2}\}_{\alpha\in [l^2]}, \{\texttt{V}_j\}_{j\in [v]})$


\FOR{ ($\alpha\gets 1, \alpha\leq l,  \alpha\gets  \alpha+1$)}
   \FOR{ ($j\gets 1, j\leq v,  j\gets  j+1$)}
    \STATE \label{linetarget1} $\mathbf{Left}_{\alpha,j} \gets A_{\alpha}* \texttt{V}_j^t*Q_{\alpha1}$

    \STATE \label{linetarget2} $\mathbf{Right}_{\alpha,j}\gets Q_{\alpha2} *\texttt{V}_j*B_{\alpha}$
    
   \ENDFOR
\ENDFOR

\STATE $m\gets o$
\FOR{ ($i\gets 1, i\leq m,  i\gets  i+1$)}
   \STATE $F_{i,VV} \gets \texttt{0}_{l\times l}$
   \FOR{ ($\alpha\gets 1, \alpha\leq l,  \alpha\gets  \alpha+1$)}
      \FOR{ ($j\gets 1, j\leq v,  j\gets  j+1$)}
         \FOR{ ($k\gets 1, k\leq v,  k\gets  k+1$)}
         \STATE  $F_{i,VV} \gets F_{i,VV}+\mathbf{Left}_{\alpha,j}*F_{i,(j,k)}^{11}*\mathbf{Right}_{\alpha,k}$
         \ENDFOR
      \ENDFOR
    \ENDFOR
      
   
\ENDFOR

 \RETURN $\{F_{i, VV}\}_{i\in [m]}$
 
\STATE \textbf{end function} 
\end{algorithmic}
\end{algorithm}



\subsection{Hamming weight model}
\label{sec:heuristic}
We analyze our attack in the \emph{Hamming weight} model, which leaks the number of ones in
the processed values. The assumption is that the power consumption of a device is correlated 
with the Hamming weights of the computed states. In our analysis, we will check whether each 
possible secret coefficient $a_i \in \{0, \ldots, 16\}$ and it leads to unique Hamming weight values during the multiplication (which 
corresponds to line $4$ or line $5$ of Algorithm~\ref{computevinegarpart}). If this is the 
case, then we expect that the leakage coming from a multiplication will allow us to identify 
the value of the secret part of vinegar values used within that multiplication. We remind the 
reader that $A_{\alpha}$, $Q_{\alpha1}$, $Q_{\alpha2}$, and $B_{\alpha}$ are public matrices, 
and we are recovering the data from the multiplication with $\texttt{V}_j$. We will analyse the Hamming 
weight of one element of the multiplication. However, it can easily extend to the entire 
multiplication without loss of generality. Moreover, since the matrix multiplication occur two 
times, the surface attack gives us a bigger chance of recovering the values of $\texttt{V}_j$.

For a first heuristic estimate, consider the \emph{expected information} that we obtain from the Hamming weight of a uniformly random $k$-bit string. Namely, $\abs{\log{\prob{\text{HW}=i}}}$ is the number of bits of information which we weigh by the probability of obtaining a state with Hamming weight $i$, leading to the expected information (or \emph{Shannon Entropy})
\[H(k):=\sum_{i=0}^k\prob{\text{ HW}=i}\cdot\abs{\log\left(\prob{\text{ HW}=i}\right)}
=\sum_{i=0}^k\frac{{k \choose i}}{2^k}\abs{\log\left(\frac{{k \choose i}}{2^k}\right)}
\]
for a uniformly random $k$-bit string.
Asymptotically, the expected information $H(k)$ grows linearly in $\sqrt{k}$. For example, we have $H(4)=1.86$ since the elements in SNOVA are represented by $4$ bits variables.

They first write a 4-bit value for multiplication of $a_1$ and $b_1$, then two 4-bit values:
\[
       H(4)+H(4) \approx 3.72
\]
bits of leakage about $a_1$ only. Since $a_1$ is a 4-bit value, it is plausible that we extract $a_1$ correctly with good probability from these operations, even if not always, since $3.72$ bits can be recovered the random variable is concentrated around its expectation rather than exactly at its expectation. 

\paragraph{Hamming weight model and Gaussian noise.}
We now add Gaussian noise with standard deviation $\sigma$ to the target trace and analyze for which $\sigma$ we can still extract one or both coefficients. Instead of searching for perfect matching, we minimize the $L_2$-norm of the \emph{differences} between the simulated target trace and the template. In our simulation with noise, we achieve $0.83$ accuracy to correct recover an element of the multiplication.  


\subsection{A side-channel attack on SNOVA}

As previously presented, Section \ref{section_rec} shows that 
an attacker only needs to recover a vector of the form $[\texttt{V}_{1,1\beta}, \ldots, \texttt{V}_{2,1\beta},\ldots , \texttt{V}_{v,l\beta}] \in \mathbb{F}_q^{lv}$ for a valid signature $(\texttt{S}, \texttt{salt})$ and some $1 \leq \beta \leq l$.  First, let us recall the values of such variables in SNOVA. 
In the official documentation, we notice that the elements 
of SNOVA lies in $\FF_q$ for $q = 16$. Implementation-wise, 
one can represent this field using only $4$ bits, and the
implementation takes such advantage and represents the 
elements in half-byte. Moreover, the implementation does not 
take into account the other $4$ bits of the byte word.

Now, there are several works that take advantage of Online Template 
Attacks (OTA) in bigger field implementations \cite{BockBBCPS24, BelaidCFGKP15},
that is, the attacks are performed on bigger fields, e.g., 
$\FF_{3329}$ or binary fields $\FF_{2^{128}}$. 

In our first attack, we will use template attacks against 
the SNOVA implementation. More precisely, we will use 
template attacks to recover partially the values of 
$\texttt{V}_{1,:\beta}, 
\ldots, \texttt{V}_{v,:\beta}$, and then use 
our recovery algorithm to recover the SNOVA private key. 

\begin{remark}
In the reference code of SNOVA, the authors perform the multiplication using tables, which allows us to target the load and store functions. However, our attack would still work even if the multiplications were performed on the fly. Additionally, while writing this paper, the authors of SNOVA made some changes to the code. Despite these changes, the leak identified in this work remains a viable attack point.
\end{remark}

\subsubsection{Attack setting.} Our setting is similar to other 
template attacks, we will perform the measurements during the 
signature procedure. In Appendix~\ref{app:code}, Listing~\ref{lst:mul} shows exactly the code part that 
we take into account to attack. In order to have a clean trace,
and have a better trigger we code the multiplication in ARM 
assembly which is then seen in Listing~\ref{lst:asm}. 

The testbed consists of a ChipWhisperer-Husky\footnote{A description is available at \url{https://www.newae.com/products/nae-cwhusky}.} board for capturing traces, and a SAM4S target board equipped with a Cortex M4 processor, 128\,KB of Flash memory, and 64\,KB of SRAM. Preliminary analysis showed that we could recover the value of the multiplication. However, the limited RAM on the SAM4S board prevents us from running the entire signing algorithm. Instead, we focused on running matrix operations extracted from real data, achieving an accuracy of $0.69$ in recovering the multiplication values. To achieve this accuracy, we required approximately 256 traces as templates, which involved performing 256 multiplications between elements of $\FF_{16}$. We are currently continuing trace acquisition and post-processing to reconstruct the targeted field elements.

